Variational Interaction Information Maximization for Cross-domain Disentanglement

Cross-domain disentanglement is the problem of learning representations partitioned into domain-invariant and domain-specific representations, which is a key to successful domain transfer or measuring semantic distance between two domains. Grounded in information theory, we cast the simultaneous learning of domain-invariant and domain-specific representations as a joint objective of multiple information constraints, which does not require adversarial training or gradient reversal layers. We derive a tractable bound of the objective and propose a generative model named Interaction Information Auto-Encoder (IIAE). Our approach reveals insights on the desirable representation for cross-domain disentanglement and its connection to Variational Auto-Encoder (VAE). We demonstrate the validity of our model in the image-to-image translation and the cross-domain retrieval tasks. We further show that our model achieves the state-of-the-art performance in the zero-shot sketch based image retrieval task, even without external knowledge. Our implementation is publicly available at: https://github.com/gr8joo/IIAE

==> method_original.tex <==
% !TEX root = neurips_2020.tex
\section{Method}
\label{headings}

Consider two domains $X$ and $Y$ that share some of the common factors in their variations. Let $Z^{S}$ be the representation space of those common factors, and $Z^{X}$ and $Z^{Y}$ be the representation spaces of the factors of domain-specific variation. We assume samples from the unknown joint data distribution $p_{D}(x,y)$, each of which is a pair 
$(x,y) \in X\times Y$ with the same shared representation $z^{s} \in Z^{S}$ and independent exclusive representations $z^{x} \in Z^{X}$ and $z^{y} \in Z^{Y}$ for each domain. Consequently, the true joint data distribution is defined as $p_{D}(x,y)=\int p_{\theta^{*}}(x|z^{x},z^{s})p_{\theta^{*}}(y|z^{y},z^{s})p_{\theta^{*}}(z^{x})p_{\theta^{*}}(z^{s})p_{\theta^{*}}(z^{y}) d z^{x} d z^{s} d z^{y}$ and the sampling processes can be elaborated by following two steps:
\begin{enumerate}
    \item Three latent factors $z^{x}$, $z^{y}$, and $z^{s}$ are independently sampled from prior distributions $p_{\theta^{*}}(z^{x})$, $p_{\theta^{*}}(z^{y})$, and $p_{\theta^{*}}(z^{s})$.
    \item Two data points $x$ and $y$ are independently sampled from the conditional distributions $p_{\theta^{*}}(x|z^{x},z^{s})$ and $p_{\theta^{*}}(y|z^{y},z^{s})$. 
\end{enumerate}
Our goal is to train a generative model that not only learns the joint distribution $p_{D}(x,y)$ by optimizing $\theta \approx \theta^*$,  but also disentangles the exclusive representations $Z^{X}$ and $Z^{Y}$ from the shared representation $Z^{S}$. We model the joint data distribution with the following VAE model that naturally reflects the assumption of independent shared / exclusive representations.
\subsection{Generative model for the joint distribution $p_{D}(x,y)$}
Let $p_{\theta}(x,y)$ be the generative model such that:
\begin{equation}
\begin{aligned}
p_{\theta}(x,y) %&= \int p_{\theta}(x,y,z) \hspace{0.2cm} d z = \int p_{\theta}(x,y,z^{x},z^{s},z^{y}) \hspace{0.2cm} d z^{x} d z^{s} d z^{y}\\
&= \int p_{\theta}(x | z^{x},z^{s}) p_{\theta}(y | z^{y},z^{s}) p_{\theta}(z^{x}) p_{\theta}(z^{s}) p_{\theta}(z^{y}) \hspace{0.2cm} d z^{x} d z^{s} d z^{y}
\end{aligned}
\end{equation}
Since the true posterior $p_{\theta}(z^{x}, z^{s}, z^{y}|x,y)=\frac{p_{\theta}(x,y,z^{x},z^{s},z^{y})}{p_{\theta}(x,y)}$ involves an intractable integration, we would like to fit it with an approximate posterior $q_{\phi}$, which is factored into three terms:
\begin{equation}
    q_{\phi}(z^{x}, z^{s}, z^{y}|x,y) = q_{x}(z^{x} | x) q_{s}(z^{s} | x, y) q_{y}(z^{y} | y)\label{eq:JointQ}
\end{equation}
\begin{figure}
    \centering
    \includegraphics[width=10cm]{figs/graphical.PNG}
    \caption{Generative model (left) and approximate posterior encoders (right).}
    \label{fig:graphical}
    \vspace{-4mm}
\end{figure}
In the following, we omit subscripts $\theta$ and $\phi$ for brevity. The graphical models of the generative model $p_{\theta}$ with the approximate posterior $q_{\phi}$ can be found in figure~\ref{fig:graphical}.
The ELBO of $p_{\theta}$ and $q_{\phi}$ can be derived as follows (full derivation in \ref{appendix:ELBO}):
\begin{equation}
\label{eq:ELBO}
\begin{aligned}
\log p(x, y) &\geq \mathbb{E}_{q(z^{x}, z^{s}, z^{y}|x,y)}\left[ \log \frac{p(x,y,z^{x},z^{s},z^{y})}{q(z^{x}, z^{s}, z^{y}|x,y)} \right]\\
&= \mathbb{E}_{q_{x}(z^{x} | x) q_{s}(z^{s} | x, y)} \left[ \log p(x | z^{x},z^{s}) \right] + \mathbb{E}_{q_{y}(z^{y} | y) q_{s}(z^{s} | x, y)} \left[ \log p(y | z^{y},z^{s}) \right]\\
&\quad - D_{KL}\left[q_{x}(z^{x} | x) \| p(z^{x})\right] - D_{KL}\left[q_{s}(z^{s} | x, y) \| p(z^{s})\right] - D_{KL}\left[q_{y}(z^{y} | y) \| p(z^{y})\right]
\end{aligned}
\end{equation}
However, maximizing this ELBO does not necessarily encourage that the representations learned by $q_{x}(z^{x} | x)$,  $q_{s}(z^{s} | x, y)$, and $q_{y}(z^{y} | y)$ are well disentangled. Specifically, the following desiderata are not reflected in the objective:
\begin{enumerate}
    \item The shared representation $Z^{S}$ should not be ignored. (All representations
    should be learned informative.)
    \item The exclusive representations $Z^{X}$ and $Z^{Y}$ should be disentangled from $Z^{S}$.
\end{enumerate}
This is mainly because we have no control over the assignment of the factors of variation to representations learned by three different encoders $q_{x}(z^{x} | x)$, $q_{s}(z^{s} | x, y)$, and $q_{y}(z^{y} | y)$. Thus, we need to devise a proper information regularization on those approximate posterior encoders for disentangled yet informative shared and exclusive representations.%$\left(z^{x} \sim q_{x}\left(z^{x}\right), z^{s} \sim q_{s}\left(z^{s}\right), z^{y} \sim q_{y}\left(z^{y}\right)\right)$

\subsection{Information regularization for disentangled representation}
All the factors of variation that underlie both of the data domains $X$ and $Y$ are the common factors that correlate the two domains. Since all those common factors should be captured in the shared representation, $Z^{S}$ is supposed to completely explain the correlation between $X$ and $Y$. This gives us motivation to learn $Z^{S}$ by maximizing $I_{q}(X;Y;Z^{S}) = I(X; Y) - I_{q}(X; Y | Z^{S})$: (see derivation in \ref{appendix:IIderivation}.) $I(X; Y)$ is constant because it is determined by the true data distribution $p_{D}(x,y)$. Thus, maximization of $I_{q}(X;Y;Z^{S})$ is equivalent to minimization of $I_{q}(X; Y | Z^{S})$. Note that $I_{q}(X; Y | Z^{S})$ is minimized to zero when $Z^{S}$ perfectly accounts for the correlation between $X$ and $Y$ so that two random variables are conditionally independent. Below we omit subscript $q$ for all entropic terms that involve with any of latent variables $z^{s}$, $z^{x}$, or $z^{y}$ for simplicity.

A desirable exclusive representation for any domain should be disentangled from the shared representation. Thus, $I(Z^{X};Z^{S})$ and $I(Z^{Y};Z^{S})$ have to be minimized. We consider the minimization of $I(Z^{X};Z^{S})$ at the moment and the other will be considered later on. By the symmetry property of interaction information, following equality always holds.
\begin{equation}
I(Z^{X}; Z^{S}) = I(Z^{X}; X) - I(Z^{X}; X | Z^{S}) + I(Z^{X}; Z^{S} | X)
\end{equation}
By \eqref{eq:JointQ}, the equality $q_{x}(z^{x}|x)=q(z^{x}|x, z^{s})$ holds. (See \ref{appendix:Integration}) Thus,
\begin{equation}
\begin{aligned}
I(Z^{X}; Z^{S} | X) &= H(Z^{X} | X) - H(Z^{X} | X, Z^{S}) = H(Z^{X} | X) - H(Z^{X} | X) = 0\\
I(Z^{X}; Z^{S}) &= I(Z^{X}; X) - I(Z^{X}; X | Z^{S})
\end{aligned}
\end{equation}

Since we want to maximize $I(X;Y;Z^{S})$ and minimize $I(Z^{X}; Z^{S})$ simultaneoulsy, we propose to optimize them together.
\begin{equation}
\begin{aligned}
&I(X;Y;Z^{S}) - I(Z^{X}; Z^{S})\\
&= I(X;Z^{S}) - I(X;Z^{S}|Y) - I(Z^{X}; X) + I(Z^{X}; X | Z^{S}) \\
&= I(X;Z^{S}) + I(Z^{X}; X | Z^{S}) - I(Z^{X}; X) - I(X;Z^{S}|Y)\\
&= H(X) - H(X|Z^{S}) + H(X|Z^{S}) - H(X|Z^{X}, Z^{S})- I(Z^{X}; X) - I(X;Z^{S}|Y)\\
&= I(X; Z^{X}, Z^{S}) - I(Z^{X}; X) - I(X;Z^{S}|Y) \\
% &\geq H(X) + \mathbb{E}_{p_{D}(x, y) q_{s}(z^{s} | x,y) q_{x}(z^{x} | x)}\left[\log p(x | z^{x}, z^{s})\right] - \mathbb{E}_{p_{D}(x,y)}\left[D_{KL}\left[ q_{x}(z^{x} | x) \| r_{x}(z^{x})\right]\right]\\
% &\quad \quad \quad \quad - \mathbb{E}_{p_{D}(x,y)}\left[D_{KL}\left[ q_{s}(z^{s} | x, y) \| r_{s}(z^{s} | y)\right]\right] \\
\end{aligned}
\end{equation}
It is quite notable that the positive entropy $H(X|Z^{S})$ originated from $- I(Z^{X}; Z^{S})$ is canceled out by the negative one from $I(X;Y;Z^{S})$. This implies that learning $Z^{S}$ uninformative to $X$, the side effect of naive minimization of $I(Z^{X}; Z^{S})$, can be compensated by maximization of $I(X;Y;Z^{S})$. Fortunately, joint optimization of those two information constraints yields $I(X; Z^{X}, Z^{S}) - I(Z^{X}; X) - I(X;Z^{S}|Y)$, which gives us an intuition about desirable objective to learn shared and exclusive representations:
\begin{enumerate}
    % \item Unlike $H(X | C)$, $H(X|Z^{S})$ is not a constant. However, it cancels out so that we do not worry about the decoder with variational distribution $p(x|z^{s})$.
    % \item $I(X;Y;Z^{S}) - I(Z^{X}; Z^{S})$ is bounded below a constant by two divergences and a reconstruction error.
    \item $I(X; Z^{X}, Z^{S})$ enforces $Z^{S}$ and $Z^{X}$ to be jointly informative to $X$.
    \item $-I(Z^{X} ; X)$ hinders $Z^{X}$ from encoding any information already encoded by $Z^{S}$, since there is no point of encoding duplicate with the cost of the amount of duplicated information penalized by the information constraint $-I(Z^{X} ; X)$.
    \item $-I(X;Z^{S}|Y)$ prevents $Z^{S}$ from encoding $X$-specific information, but does not penalize encoding shared representation. This is because it is an information constraint that differentiates the type of the information encoded by $Z^{S}$. As long as $Z^{S}$ extracted from $X$ underlies in $Y$ as well, $Z^{S}$ is conditionally uninformative to $X$ and makes $I(X;Z^{S}|Y)$ zero.
\end{enumerate}

% Repeating the same process to $Y$, we also achieve:
% \begin{equation}
% \begin{aligned}
% &I(X;Y;Z^{S}) - I(Z^{Y}; Z^{S}) = I(Y; Z^{Y}, Z^{S}) - I(Z^{Y}; Y) - I(Y;Z^{S}|X) \\
% &\geq H(Y) + \mathbb{E}_{p_{D}(x, y) q_{s}(z^{s} | x,y) q_{x}(z^{x} | x)}\left[\log p(y | z^{y}, z^{s})\right] - \mathbb{E}_{p_{D}(x,y)}\left[D_{KL}\left[ q_{y}(z^{y} | y) \| p(z^{y})\right]\right]\\
% &\quad \quad \quad \quad - \mathbb{E}_{p_{D}(x,y)}\left[D_{KL}\left[ q_{s}(z^{s} | x, y) \| r_{s}(z^{s} | x)\right]\right]
% \end{aligned}
% \end{equation}
Repeating the same process to $Y$, we also achieve another information constraint $I(X;Y;Z^{S}) - I(Z^{Y}; Z^{S})$. The lower bound on the summation of those two information constraints, $I(X;Y;Z^{S}) - I(Z^{X}; Z^{S})$ and $I(X;Y;Z^{S}) - I(Z^{Y}; Z^{S})$, yields an objective function similiar to the ELBO with subtle difference.
\begin{equation}
\label{eq:InfoConst}
\begin{aligned}
&2 \cdot I(X;Y;Z^{S}) - I(Z^{X};Z^{S}) - I(Z^{Y};Z^{S}) \\
&= I(X; Z^{X}, Z^{S}) + I(Y; Z^{Y}, Z^{S}) - I(Z^{X}; X) - I(Z^{Y}; Y) - I(Y;Z^{S}|X) - I(X;Z^{S}|Y)\\
&\geq \mathbb{E}_{p_{D}(x, y) q_{s}(z^{s} | x,y) p_{x}(z^{x} | x)}\left[\log p(x | z^{x}, z^{s})\right] + \mathbb{E}_{p_{D}(x, y) q_{s}(z^{s} | x,y) q_{x}(z^{x} | x)}\left[\log p(y | z^{y}, z^{s})\right]\\
&\quad - \mathbb{E}_{p_{D}(x,y)}\left[D_{KL}\left[ q_{x}(z^{x} | x) \| q_{x}(z^{x})\right]\right] - \mathbb{E}_{p_{D}(x,y)}\left[D_{KL}\left[ q_{y}(z^{y} | y) \| p(z^{y})\right]\right]\\
&\quad - \mathbb{E}_{p_{D}(x,y)}\left[D_{KL}\left[ q_{s}(z^{s} | x, y) \| r^{y}_{s}(z^{s} | y)\right]\right] - \mathbb{E}_{p_{D}(x,y)}\left[D_{KL}\left[ q_{s}(z^{s} | x, y) \| r^{x}_{s}(z^{s} | x)\right]\right]\\
&\quad + H(X) + H(Y)\\
\end{aligned}
\end{equation}
The inequality is proved in \ref{appendix:InfoConst}. Ignoring constant entropy terms $H(X)$ and $H(Y)$, this lower bound can be also obtained from the ELBO with substituting
$D_{KL}\left[ q_{s}(z^{s} | x, y) \| r^{y}_{s}(z^{s} | y)\right] + D_{KL}\left[ q_{s}(z^{s} | x, y) \| r^{x}_{s}(z^{s} | x)\right]$ for $D_{KL}\left[q_{s}(z^{s} | x, y) \| p(z^{s})\right]$. Since $\mathbb{E}_{p_{D}(x,y)}\left[D_{KL}\left[q_{s}(z^{s} | x, y) \| p(z^{s})\right]\right]$ is an upper bound on $I(Z^{S};X,Y)$, it can be considered as an information constraint on the shared representation which penalizes the amount of information without differentiating if $z^{s}$ encoded shared or domain specific information. On the other hand, $\mathbb{E}_{p_{D}(x,y)}\left[D_{KL}\left[ q_{s}(z^{s} | x, y) \| r^{y}_{s}(z^{s} | y)\right]\right] + \mathbb{E}_{p_{D}(x,y)}\left[D_{KL}\left[ q_{s}(z^{s} | x, y) \| r^{x}_{s}(z^{s} | x)\right]\right]$, an upper bound on $I(X;Z^{S}|Y) + I(Y;Z^{S}|X)$, penalizes only the amount of domain specific information. Furthermore, they naturally introduce variational encoders $r^{x}_{s}(z^{s} | x)$ and $r^{y}_{s}(z^{s} | y)$.

\subsection{Interaction Information Autoencoder}
We want to train a generative model with the ELBO defined in eq.\ref{eq:ELBO} under the constraint to keep the information regularization terms defined in eq.\ref{eq:InfoConst} to be maximal. However, the constrained optimization is relatively difficult to optimize. Thus, we relax the information constraint by allowing the model to maximize it jointly with the ELBO as done in a similar way in \citep{moyer2018invariant}. The resulting final objective function is following:
% \begin{equation}
% \max \mathbb{E}_{x, y}\left[\log p_{\theta}(x,y)\right] +\lambda \left(2 \cdot I(X;Y;Z^{S}) - I(Z^{X};Z^{S}) - I(Z^{Y};Z^{S}) \right)
% \end{equation}
\begin{equation}
\begin{aligned}
%&\max \mathbb{E}_{p_{D}(x, y)}\left[\log p_{\theta}(x,y)\right]
&\max_{p,q} \mathbb{E}_{q(z^{x}, z^{s}, z^{y}|x,y)}\left[ \log \frac{p(x,y,z^{x},z^{s},z^{y})}{q(z^{x}, z^{s}, z^{y}|x,y)} \right] + \lambda \left(2 \cdot I(X;Y;Z^{S}) - I(Z^{X};Z^{S}) - I(Z^{Y};Z^{S}) \right)\\
&\geq \max_{p,q,r} \left(1+\lambda \right) \cdot \mathunderline{blue}{ \mathbb{E} \left[\hspace*{0.1cm} \mathbb{E}_{q_{x}(z^{x} | x) q_{s}(z^{s} | x,y)} \left[ \log p(x | z^{x},z^{s}) \right] + \mathbb{E}_{q_{y}(z^{y} | y) q_{s}(z^{s} | x,y)} \left[ \log p(y | z^{y},z^{s}) \right] \hspace*{0.1cm}\right] }\\
&\quad \quad \quad - \left(1+\lambda \right) \cdot \mathunderline{blue}{\mathbb{E} \left[\hspace*{0.1cm} D_{KL}\left[q_{x}(z^{x} | x) \| p(z^{x})\right] + D_{KL}\left[ q_{y}(z^{y} | y) \| p(z^{y}) \right] \hspace*{0.1cm} \right] }\\
&\quad \quad \quad - \mathunderline{green}{\mathbb{E} \left[ \hspace*{0.1cm} D_{KL}\left[ q_{s}(z^{s} | x, y) \| p(z^{s})\right] \hspace*{0.1cm} \right] }\\
&\quad \quad \quad - \lambda \cdot \mathunderline{red}{\mathbb{E} \left[ \hspace*{0.1cm} D_{KL}\left[ q_{s}(z^{s} | x, y) \| r_{s}^{y}(z^{s} | y) \right] + D_{KL}\left[ q_{s}(z^{s} | x, y) \| r_{s}^{x}(z^{s} | x) \right] \hspace*{0.1cm} \right] }\\
\end{aligned}
\end{equation}
Terms with blue underline are from both ELBO and information constraints, green from only the ELBO, and red from only the information constraints. In order to maximize this lower bound, we propose the model named Interaction Information AutoEncoder (IIAE) that can be found in figure \ref{fig:IIAE}.

\begin{wrapfigure}{r}{7cm}
\caption{Network structure of IIAE}
\label{fig:IIAE}
\includegraphics[width=7cm]{figs/IIAE.PNG}
\vspace{-4mm}
\end{wrapfigure} 
%------------------------------------------
% \lipsum[2-3]
% \par
% Figure~\ref{fig:IIAE} is a wrapped figure.


% \begin{figure}
%     \centering
%     \includegraphics[width=8cm]{figs/IIAE.PNG}
%     \caption{Proposed model}
%     \label{fig:IIAE}
% \end{figure}
